An In-depth Study on Internal Structure of Chinese Words

Unlike English letters, Chinese characters have rich and specific meanings. Usually, the meaning of a word can be derived from its constituent characters in some way. Several previous works on syntactic parsing propose to annotate shallow word-internal structures for better utilizing character-level information. This work proposes to model the deep internal structures of Chinese words as dependency trees with 11 labels for distinguishing syntactic relationships. First, based on newly compiled annotation guidelines, we manually annotate a word-internal structure treebank (WIST) consisting of over 30K multi-char words from Chinese Penn Treebank. To guarantee quality, each word is independently annotated by two annotators and inconsistencies are handled by a third senior annotator. Second, we present detailed and interesting analysis on WIST to reveal insights on Chinese word formation. Third, we propose word-internal structure parsing as a new task, and conduct benchmark experiments using a competitive dependency parser. Finally, we present two simple ways to encode word-internal structures, leading to promising gains on the sentence-level syntactic parsing task.

==> content/TODO.tex <==



赛豪：对于包含特殊字符的词，一些有规律的词，不能光靠人去标，可以用规则确定其内部结构。

利用上下文信息做词内部结构

利用字义、词义解释（例句）等，来做词内部结构

字义、词义资源的获取、整理、标注



==> content/_not-used-exp.tex <==
% 实验的抓紧做，把主要结果做出来。

% 1）只出现在dev/test中的词，用预测的内部结构，结果如何？2）字级别句法分析的结果如何？比规则的波浪形的结果如何？

% 句法用CRF-loss（一阶）的结果也应该跑一下，我们起码自己要知道结果。

% 句法用BERT时，词内部结构是否还有用？可以看看，自己看看结果。

% 字内部时用了BERT，现在不用的话，也不好。

\section{Experiments}
\textbf{Data.}
For the task of char-level syntactic parsing for words, we use our manually annotated char-level syntactic treebank, which consists of xxx, xxx, and xxxx words in training, development, and test sets respectively. For sentence-level syntactic parsing, we conduct experiments and analysis on the Chinese Penn Treebank 5.0 (CTB5) with dependencies obtained by the Penn2Malt tool \footnote{http://stp.lingfil.uu.se/∼nivre/research/Penn2Malt.html} and the Chinese data at the
CoNLL09 shared task \citet{conll09}. We adopt the same data split as \citet{zhang-clark-2008} on CTB5 and the gold standard data split on CoNLL09. 

For pretrained char embeddings and word embeddings, we adopt the 100 dimension embeddings of \citet{liying-2019} pretrained with word2vec model on Chinese Gigaword.

\textbf{Evaluation metrics.} 
We use the standard unlabeled and labeled attachment score (UAS/LAS) as the main metrics for both char-level syntactic parsing and sentence-level syntactic parsing.

\textbf{Model settings.} 
We adopt most of the parameter settings in Biaffine parser \cite{dozat2016deep}. Each model is
trained for at most 1000 iterations.
We stop training when the peak performance
on the development data does not increase in 100 consecutive iterations. 
We set the dimensions of char embedding, word
embedding, and CharLSTM outputs to 50, 100, 100, respectively. 

\subsection{Results: Word-internal Syntactic Parsing}
\setlength{\tabcolsep}{5pt}
\begin{table}[tb]
%\setlength{\leftskip}{-25pt}
\begin{center}
\begin{small}
\begin{tabular}{c | *{2}{c}  | *{2}{c} }
\hline
\multirow{2}{*}{} 
& \multicolumn{2}{|c}{dev }
& \multicolumn{2}{|c}{test} \\
\cmidrule(lr){1-2} \cmidrule(lr){4-5}
% \cline{2-3} \cline{4-5}
& UAS & LAS & UAS & LAS \\
\hline
Random & 78.85 & 73.93  & 79.17 & 74.21 \\
%\hline
Pretrained & 80.07 & 75.45 & 79.74 & 75.00 \\
%\hline
BERT & 86.42 & 83.39 & 86.48 & 83.35 \\
\hline
\end{tabular}
\end{small}
\caption{Results of word-internal syntactic parsing.}
\label{iwdp-result}
\end{center}
\end{table}

Table \ref{iwdp-result} presents the results of word-internal parsing. 




1)随机<pretrain<bert
2)用词性比不用词性的结果好
% We observe that the pretrained embedding 


% leads to consistent and large improvement on both domains. Compared with
% “ELMo (Giga)”, LAS increases b

% The comparison between pretrained embeddings and randomly initialized embeddings
% shows that both pretrained embeddings and lexicon are useful to lattice LSTM, and lexicon contributes more than the
% pretrained embeddings

黄：adv和的模型预测准确率较低的原因，可能是因为adv标签容易和coo标签混淆，如果某个词是由几个动词性字组成的话，那么模型可能会比较难判断出来这两个动词性字之间是修饰关系还是并列关系。
通过观察预测结果发现，adv确实容易和coo混淆，还有和att和混淆。



\begin{figure}
		\centering
		\includegraphics[scale=0.3]{figure/model-acc.png}
		\caption{xxxx【图要重画】}
		\label{fig:model-acc}
\end{figure}



==> content/abstract-old.tex <==
    \begin{abstract}

Unlike English letters, Chinese characters have rich and specific meanings. Usually, the meaning of a word can be derived from its constituent characters in some way. 
Several previous works on syntactic parsing propose to annotate shallow word-internal  structures for better utilizing character-level information. 
%Many previous studies try to model and utilize word-formation laws for better word understanding and representation. 
%Different from most Indo-European languages such as English, Chinese characters convey meanings, and the meaning of most words are derived from their constituent characters.
This work proposes to model the deep internal structures of Chinese words as dependency trees with 11 labels for distinguishing syntactic relationships. 
%We endeavour to answer three questions. 1) What are 
%the word-formation laws for Chinese words? 2) How well can a model be trained to predict deep word-internal structures? 
%3) Is modeling word-internal structures beneficial for word representations? 
%Specifically, this work can be decomposed into four parts. 
First, based on newly compiled annotation guidelines, we 
%based on linguistic textbooks and sentence-level syntactic annotation projects.
manually annotate a word-internal structure treebank (WIST) consisting of over 30K multi-char words from Chinese Penn Treebank. 
To guarantee quality, each word is independently annotated by two annotators and inconsistencies are handled by a third senior annotator.  
Second, we present detailed and interesting analysis on WIST to reveal insights on Chinese word formation. 
Third, we propose word-internal structure parsing as a new task, and conduct benchmark experiments using a competitive dependency parser. 
Finally, we present two simple ways to encode word-internal structures, leading to promising gains on %and show that such structure-aware word representations is beneficial for 
the sentence-level syntactic parsing task. 
% 有点长，还要凝练。questions考虑放到introductions中


% Typically, words are considered as the basic semantic units for Chinese language processing and therefore the representation of words becomes a core issue. Previous work usually represents words by considering their contextual information or encode the constituent characters of words with the assumption that each word has a flat structure.
% Such word representations give no consideration to char-level syntactic structures for words, an informative linguistic source that can reflect the dependency relations between characters and convey meanings to alleviate out-of-vocabulary issues.
% In this work, we conduct an in-depth study on char-level syntactic structures. First, we manually annotate over xxx words with char-level syntactic structures according to our newly compiled annotation guideline and give detailed analysis to gain more
% insights on the construction of Chinese words.
% Then, we propose to parse the structures with a simple yet effective graph-based parser. Finally, by applying intra-word structures to two downstream tasks, i.e., word-based and char-based dependency parsing, we verify the effectiveness of intra-word character dependency structures and its potential capability in better understanding deeper level information of Chinese words. 

% Motivation两方面：
% 1）汉语中字有明确的含义，古代的时候单字词占绝大多数。由字到词的规律（即构词法）非常有趣，对于新词发现和理解应该也会很有帮助。
% 2）目前深度学习下，三种主流词表示方法：word emb, charLSTM（序列，不考虑深层次的字间关系），上下文相关表示，均没有考虑词内部结构。

\end{abstract}



% 龚晨：先不着急写abstract。先把要写的东西，乱七八糟的写出来，放在intro，最后根据实验结果再去梳理，再决定怎么讲故事。
% Traditionally, natural language processing tasks for Chinese language usually consider words or characters as basic linguistic units. On the one hand, word-based method preserves more semantic information. However（不是连词，这时两句话）, due to the flexibility of Chinese word construction, it is not easy for the model to accurately learn word semantics, especially for those out-of-vocabulary words. On the other hand, although character-based method can alleviate data sparseness issue, it is prone to suffer from ambiguity problem.
% In this paper, we investigate character-level dependency structure（尝试采用依存树来刻画词语的构成、构词法、构词法的翻译？word-building word-formation？ ） to capture the internal syntactic relations for words, a linguist source which contains richer syntax and semantic information than characters and is less sparse than words.
% 我感觉我们要把意义讲大一些。光是针对汉语构词法的研究，就很有意义了。
% First, we manually annotate over xxx words with intra-word character dependency structures according to our newly compiled annotation guideline. Then, we propose to parse intra-word character dependency by employing a simple yet effective graph-based parser. Finally, by 
% applying intra-word character dependency trees to two downstream tasks, i.e., word-based dependency parsing and semantic role labeling, we verify the effectiveness of intra-word character dependency structures and its potential capability in better understanding deeper level information of Chinese words. 

% 构词法研究的意义：更好的词表示；更好的词义理解；新词发现；新词的含义理解

==> content/extended-charlstm.tex <==
\subsection{Representation with BiLSTM}
% \textbf{Encoding with sequence model.}
Apart from the novel graph neural network, we also utilize CharLSTM, without changing the major network structure of baseline model, to integrate structure-aware word representations.
% 除了使用新颖的图神经网络之外，我们还给出另外一个十分直接的引入字结构表示信息的方法，which 我们不需要引入别的神经网络结构。
% 师姐我说我们用charLSTM编码label的初衷是，
% In syntactic parsing task, one of the most important role of the CharLSTM is to explore the part-of-speech clues of a word from characters it contained.
% For Chinese language, 【可以说，中心词以及非中心字的语法角色隐含了词性信息吗? 比如``枣红''的中心字是``红''，而``红枣''的中心字是``枣''】.
As depicted in Table \ref{table:summary-different-num-word}, about $92.1\%$ words in the dataset are one-character words or two-character words.
Their word-internal skeleton trees are simple, but the word-internal dependency labels still can provide clues. We encode such dependency label information by employing a BiLSTM.
% by pointing out center-character and illustrating the function of non-center-characters.
% So, we omit the arcs of the word-internal structures.
% , and feed each character together with its relation labels into the CharLSTM.
% That is, for now, the input of CharLSTM in Equation \ref{baseline-input} is $w_i$ and $l_{u,v}$, the label of dependency $u \leftarrow v$. 【这里的的公式还有些奇怪，得再改一下】
% 在依存解析中，charLSTM的一个很重要的任务是去从组成词的字中发掘POS信息。我们发现基于这个出发点 词内部的每个字的label要比字符间的依存弧更为重要，因为它可以指出哪个字为词语的中心字并标明不同字在词语中所承担的角色。因此我们为了使得模型更加简单而忽略arc。
Formally, we concatenate the character embedding with the dependency label embedding, and then go through a single-layer BiLSTM:
\begin{equation}
    % [\overrightarrow{\mathbf{h}}_{u}, \overleftarrow{\mathbf{h}}_{u} ] =\textup{BiLSTM}(\mathbf{emb}^{c}(c_u) \oplus \mathbf{emb}^{l}(l_{u,v}))
    {\mathbf{h}}_{u} =\textup{BiLSTM}(\mathbf{emb}^{c}(c_u) \oplus \mathbf{emb}^{l}(l_{u,v}))
\end{equation}
Here, $\mathbf{emb}^{l}(l_{u,v})$ is the label embedding for dependency $u \leftarrow v$.
The pooling operation is performed on the top-layer ouputs of BiLSTM to obtain $\mathbf{r}_i^{syn}$, which is the same as Equation \ref{pooling}. 
% The final syntactic structure-aware representation $\mathbf{r}_i^{syn}$ 
% The final representation $\mathbf{r}_i^{syn}$ is the concatenation of $\overrightarrow{\mathbf{h}}_{n}$, the forward hidden representation of the last word of the sentence, and $\overleftarrow{\mathbf{h}}_{0}$, the backward representation of the first word.
% The final representation $\mathbf{r}_i^{syn}$ is the top-layer BiLSTM outputs.





% In addition to directly encoding the syntactic word-internal tree structure with the graph model GCN, we also employ the sequence model BiLSTM to obtain the structure-aware word representation.


==> figure/barchart-label-acc.tex <==
\begin{figure}[tb]
  \begin{tikzpicture}
    \begin{axis} [
        width=8.6cm, height=4.5cm,
        ybar,
        axis y line=left,
        axis x line=left,
        x axis line style={-},
        ymajorgrids=true,
        enlarge x limits=0.06,
        tick align=outside,
        ymin=55, ymax=92,
        symbolic x coords={
            root, att, coo, frag, obj, adv, cmp, adjct, subj, repet, pobj
        },
        xtick=data,
        nodes near coords=\pgfmathprintnumber\pgfplotspointmeta,
        xticklabel shift=6,
        x tick label style={anchor=base, font=\scriptsize},
        y tick label style={font=\scriptsize},
    ]
    \addplot [
        draw=black,
        fill opacity=0.2, 
        text opacity=1,
        font=\tiny, 
        fill={rgb,255:red,76; green,114; blue,176}] coordinates {
        (root, 89.03)
        (att, 89.46)
        (coo, 75.77)
        (frag, 80.6)
        (obj, 77.4)
        (adv, 68.03)
        (cmp, 84.04)
        (adjct, 76.76)
        (subj, 64.17)
        (repet, 81.08)
        (pobj, 58.06)
    };
  \end{axis}
\end{tikzpicture}

\caption{
  Accuracy on different dependency labels.
}
\label{fig:model-acc}
\end{figure}

